Convergence Rates of Stochastic Zeroth-order Gradient Descent for \L ojasiewicz Functions

We prove convergence rates of Stochastic Zeroth-order Gradient Descent (SZGD) algorithms for Lojasiewicz functions. The SZGD algorithm iterates as \begin{align*} \mathbf{x}_{t+1} = \mathbf{x}_t - \eta_t \widehat{\nabla} f (\mathbf{x}_t), \qquad t = 0,1,2,3,\cdots , \end{align*} where $f$ is the objective function that satisfies the \L ojasiewicz inequality with \L ojasiewicz exponent $\theta$, $\eta_t$ is the step size (learning rate), and $ \widehat{\nabla} f (\mathbf{x}_t) $ is the approximate gradient estimated using zeroth-order information only. Our results show that $ \{ f (\mathbf{x}_t) - f (\mathbf{x}_\infty) \}_{t \in \mathbb{N} } $ can converge faster than $ \{ \| \mathbf{x}_t - \mathbf{x}_\infty \| \}_{t \in \mathbb{N} }$, regardless of whether the objective $f$ is smooth or nonsmooth.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Example Article\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> tex/archive.tex <==
----------------------------------

Now let's consider the following setting: 
\begin{itemize}
    \item The objective function $f$ is $L$-smooth: $ \| \nabla f (z) - \nabla f (z')\| \le L \| z - z' \| $ for all $z,z' \in \R^n$. 
    \item The objective function $f$ satisfies the (global) PL condition: 
    \begin{align*} 
        \frac{1}{2} \| \nabla f (x) \|^2 \ge \mu \( f (x) - f^* \) , \qquad \forall x \in \R^n, 
    \end{align*} 
    where $ f^* > -\infty $ is the global minimum of $f$. 
    \item Consider a stochastic process $ \{ x_t \}_{t \ge 1} $ ($x_t \in \R^n$), and let $ \F_t $ be the $\sigma$-algebra generated by $x_1, x_2, \cdots, x_t$. 
    \item The stochastic process $\{x_t\}_{t \ge 1}$ is described by a stochastic gradient descent process: 
    \begin{align*}
        x_{t+1} = x_t - \eta w_t, \qquad \forall t \ge 1
    \end{align*} 
    where 
    \begin{align*}
        \E \[ w_t | \F_t \] = \nabla f (x_t) , \qquad \E \[ \| w_t \|^2 | \F_t \] \le \alpha \|  \nabla f (x_t) \|^2, 
    \end{align*}
    for some constant $\alpha$. 
\end{itemize} 

\textcolor{red}{Note that our gradient estimator is approximately $w_t$. }

By $L$-smoothness, we immediately have the following: 
\begin{align*}
    f (x_{t+1}) 
    \le& \; 
    f (x_t) - \eta \nabla f (x_t)^\top w_t + \frac{\eta^2 L}{2} \| w_t \|^2. 
\end{align*}

Taking conditional expectation and setting $\eta = \frac{1}{\alpha L}$, we get
\begin{align*}
    \E \[ f (x_{t+1})  | \F_t \]
    \le 
    f (x_t) - \frac{1}{2 \alpha L} \| \nabla f (x_t) \|^2 
    \le 
    \frac{\mu}{ \alpha L } \( f (x_t) - f^* \),  
\end{align*} 
where the last inequality follows from the PL condition. 


Thus we have 
\begin{align*} 
    \E \[ f (x_{t+1}) - f^* | \F_t \] \le \( 1 - \frac{\mu}{\alpha L} \) \( f (x_t) - f^* \) . 
\end{align*} 

For simplicity, let $\beta = 1 - \frac{\mu}{\alpha L} $ and let $y_t = f (x_t) - f^*$. 

Seems that we already have a linear convergence result (in expectation): 
\begin{align*}
    \E \[ y_{t+1} \] 
    =& \; 
    \E \[ \E \[ y_{t+1} | \F_t \] \] \\
    % =& \; 
    \le& \; 
    \beta \E \[ y_t \]  \\
    \le& \; 
    \cdots \\
    \le& \; 
    \beta^t y_0. 
\end{align*}
% Next we will target at the stochastic process $ \{ y_{t+1} - \beta y_t \}_{t \ge 1} $, which is a supermartingale difference sequence. 

-----------------------------------------------------------

\textcolor{red}{Almost sure convergence} 

Fix any $\epsilon \in \( 0, \frac{1}{\beta} - 1 \)$. Consider the sequence $\left\{ \( \frac{1}{\beta} - \epsilon \)^t y_{t+1}  \right\}_{t \in \mathbb{N}}$. 

By Markov inequality, we have 
\begin{align*} 
    \Pr \(  \( \frac{1}{\beta} - \epsilon \)^t y_{t+1}  \ge \delta \) 
    \le 
    \frac{ \( \frac{1}{\beta} - \epsilon \)^t \E \[ y_{t+1} \] }{ \delta }
    \le 
    \frac{ \( 1 - \epsilon \beta \)^t }{ \delta } . 
\end{align*} 

Let $ Z_t :=  \( \frac{1}{\beta} - \epsilon \)^t y_{t+1} $. 


Let $\delta$ be an arbitrary positive number. Let $ \{ s_1, s_2, \cdots \} $ be a subsequence of $\{ 0,1,2,\cdots \}$. Note that the events $ \{ Z_{s_k} \ge \delta \} $ are contained in the sample space generated by the stochastic gradient descent process. We have, by Markov inequality, 
\begin{align*} 
    \Pr \( Z_{t} > \delta \text{ infinitely often} \) 
    \le 
    \lim_{k \rightarrow \infty } \frac{ \( 1 - \epsilon \beta \)^{s_k} }{ \delta } = 0 .       
\end{align*} 

Since the events $ \{ Z_{t} > \delta \text{ infinitely often} \} $ increases as $\delta$ decreases, we have 
\begin{align*} 
    \left\{ \lim_{t \rightarrow \infty } Z_t = 0 \right\}^c 
    = 
    \bigcup_{\delta > 0} \{ Z_{t} > \delta \text{ infinitely often} \} 
    = 
    \bigcup_{\delta \in \mathbb{Q}_+ } \{ Z_{t} > \delta \text{ infinitely often} \} , 
\end{align*} 
where we replace the union over an uncountable set with a union over a countable set. 


Thus it holds that 
\begin{align*} 
    1 - \Pr \( \lim_{t \rightarrow \infty} Z_t = 0 \) 
    =& \;  
    \Pr \( \bigcup_{\delta \in \mathbb{Q}_+ } \{ Z_{t} > \delta \text{ infinitely often} \}  \) \\
    \le& \; 
    \sum_{\delta \in \mathbb{Q}_+} \Pr \( Z_{t} > \delta \text{ infinitely often} \) \\
    =& \; 
    0 , 
\end{align*}
which shows that $Z_t$ converges to zero with probability 1. 

% $ \mathcal{E}_t := \left\{  \ge \frac{1}{t} \right\} $. 

-------------------------------------------------------

\textcolor{red}{more formal writeup}

==> tex/convergence.tex <==


\section{Algorithm and Convergence Rate} 



Consider the gradient descent algorithm with estimated gradient: 
\begin{align} 
    x_{t+1} = x_t - \eta_t \wh{\nabla} f (x_t), \qquad t = 0,1,2,\cdots , \label{eq:gd}
\end{align} 
where $ \wh{\nabla} f (x_t) $ is a gradient estimator of $f$ at $x_t$, and $\eta_t > 0$ is the step size (learning rate) at $t$. 

estimation tasks in $\R^n$. 
The gradient estimator is: 
\begin{align} 
    \wh{\nabla} f_k^\delta (x) := \frac{n}{2 \delta k} \sum_{i=1}^k \( f ( x + \delta v_i ) - f (x - \delta v_i) \) v_i, \quad \forall x \in \R^n, \label{eq:def-grad-est}
\end{align} 
where $ [v_1, v_2, \cdots, v_k] $ is uniformly sampled from the Stiefel's manifold $ \text{St} (n,k) $, and $\delta$ is the finite difference granularity. 

\begin{definition}
    \label{def:smooth}
    A function $f : \R^n \rightarrow \R$ is called $ (k,L) $-smooth ($k \in \mathbb{N}_+$, $L > 0$) if it is $k$-times continuously differentiable, and 
    \begin{align*} 
        \| \partial^{k-1} f (x) - \partial^{k-1} f (x') \| \le L \| x - x' \|, \quad \forall x,x' \in \R^n, 
    \end{align*}  
    where $\partial^{k-1} f (x) $ is the $(k-1)$-th total derivative of $f$ at $x$, and $ \| \cdot \| $ is the spectral norm when applied to symmetric multi-linear forms and the Euclidean norm when applied to vectors. 
    % on the left hand side, the  
    The spectral norm of a symmetric multi-linear form $F$ is $ \| F \| : = \sup_{ v\in\R^n, \| v \| = 1 } F[v] $. 
\end{definition} 

\begin{theorem}
    If $f$ is $(3,L_3)$-smooth, the variance of the gradient estimator for $f$ satisfies 
    \begin{align*} 
        &\; \E \[ \left\| \wh{\nabla}  f_k^\delta (x) - \E \[ \wh{\nabla}  f_k^\delta (x) \] \right\|^2 \] \\
        \le& \;  
        \( \frac{n}{k}  - 1 \) \| \nabla f (x) \|^2 + \frac{L_3 \delta^2}{3} \( \frac{n^2}{k}  - n \) \| \nabla f (x) \| + \frac{L_3^2 n^2 \delta^4 }{36 k } , \quad \forall x \in \R^n. 
    \end{align*} 
\end{theorem}
